Deep learning for understanding multilabel imbalanced Chest X-ray datasets

Over the last few years, convolutional neural networks (CNNs) have dominated the field of computer vision thanks to their ability to extract features and their outstanding performance in classification problems, for example in the automatic analysis of X-rays. Unfortunately, these neural networks are considered black-box algorithms, i.e. it is impossible to understand how the algorithm has achieved the final result. To apply these algorithms in different fields and test how the methodology works, we need to use eXplainable AI techniques. Most of the work in the medical field focuses on binary or multiclass classification problems. However, in many real-life situations, such as chest X-rays, radiological signs of different diseases can appear at the same time. This gives rise to what is known as "multilabel classification problems". A disadvantage of these tasks is class imbalance, i.e. different labels do not have the same number of samples. The main contribution of this paper is a Deep Learning methodology for imbalanced, multilabel chest X-ray datasets. It establishes a baseline for the currently underutilised PadChest dataset and a new eXplainable AI technique based on heatmaps. This technique also includes probabilities and inter-model matching. The results of our system are promising, especially considering the number of labels used. Furthermore, the heatmaps match the expected areas, i.e. they mark the areas that an expert would use to make the decision.

==> tablas_novalidas.tex <==
\begin{table}[H]
\caption{Result obtained from the ensemble with specific labels, including results from each architecture.}
\label{tab:result_general}
\resizebox{\textwidth}{!}{\begin{tabular}{r|lllll|l|l} \toprule
                               & DenseNet 201    & efficientNet B0 & Inception       & InceptionResnet & Xception        & ensemble        & Nº samples \\ \midrule \midrule
Normal                         & 0,8197          & 0,8114          & \textbf{0,8318} & 0,8204          & 0,8270          & \textit{0,8375} & 34327.0    \\
Copd signs                     & \textbf{0,8229} & 0,7847          & 0,8163          & 0,8147          & 0,7996          & \textit{0,8326} & 13419.0    \\
Cardiomegaly                   & \textbf{0,9268} & 0,9067          & 0,9263          & 0,9267          & 0,9217          & \textit{0,9366} & 8412.0     \\
Aortic elongation              & 0,8846          & 0,8463          & 0,8823          & \textbf{0,8879} & 0,8878          & \textit{0,8938} & 1399.0     \\
Unchanged                      & 0,6363          & 0,6140          & 0,6380          & \textbf{0,6420} & 0,6360          & \textit{0,6411} & 1311.0     \\
Scoliosis                      & 0,7588          & 0,7116          & 0,7453          & 0,7323          & \textbf{0,7740} & \textit{0,7931} & 1073.0     \\
Chronic changes                & 0,7592          & 0,7201          & \textbf{0,7682} & 0,7625          & 0,7524          & \textit{0,7723} & 873.0      \\
Costophrenic angle blunting    & \textbf{0,8620} & 0,8447          & 0,8323          & 0,8306          & 0,8546          & \textit{0,8770} & 703.0      \\
Air trapping                   & \textbf{0,6919} & 0,6866          & 0,5150          & 0,4693          & 0,5060          & \textit{0,7038} & 663.0      \\
Pneumonia                      & 0,8150          & 0,8208          & 0,8101          & \textbf{0,8214} & 0,8206          & \textit{0,8499} & 651.0      \\
Pleural effusion               & \textbf{0,9593} & 0,9514          & 0,9558          & 0,9553          & 0,9452          & \textit{0,9665} & 658.0      \\
Interstitial pattern           & 0,8340          & 0,8276          & \textbf{0,8457} & 0,8434          & 0,8302          & \textit{0,8576} & 594.0      \\
Infiltrates                    & 0,8118          & 0,8032          & 0,8033          & \textbf{0,8152} & 0,8077          & \textit{0,8396} & 591.0      \\
Vertebral degenerative changes & 0,7791          & 0,7298          & 0,7743          & \textbf{0,7847} & 0,7793          & \textit{0,7971} & 575.0      \\
Laminar atelectasis            & \textbf{0,8426} & 0,8121          & 0,8273          & 0,8271          & 0,8331          & \textit{0,8580} & 578.0      \\
Kyphosis                       & \textbf{0,8669} & 0,8340          & 0,8452          & 0,8487          & 0,8392          & \textit{0,8697} & 526.0      \\
Vascular hilar enlargement     & 0,7464          & 0,7419          & \textbf{0,7689} & 0,7548          & 0,7445          & \textit{0,7831} & 463.0      \\
Apical pleural thickening      & \textbf{0,8080} & 0,8007          & 0,7888          & 0,5086          & 0,5005          & \textit{0,8305} & 469.0      \\
Fibrotic band                  & \textbf{0,8306} & 0,8087          & 0,8133          & 0,5750          & 0,8065          & \textit{0,8483} & 449.0      \\
Nodule                         & \textbf{0,7061} & 0,6745          & 0,5613          & 0,5744          & 0,5506          & \textit{0,7042} & 449.0      \\
Calcified granuloma            & \textbf{0,8085} & 0,8021          & 0,5418          & 0,5542          & 0,4961          & \textit{0,8329} & 388.0      \\
Callus rib fracture            & 0,7168          & \textbf{0,7648} & 0,6139          & 0,6085          & 0,5709          & \textit{0,7875} & 360.0      \\
Pacemaker                      & 0,9933          & \textbf{0,9972} & 0,9961          & 0,9961          & 0,9839          & \textit{0,9973} & 336.0      \\
Aortic atheromatosis           & 0,8564          & 0,8471          & 0,8619          & 0,8518          & \textbf{0,8710} & \textit{0,8848} & 318.0      \\
Bronchiectasis                 & 0,8006          & 0,7751          & 0,7964          & \textbf{0,8048} & 0,7942          & \textit{0,8203} & 290.0      \\
Sternotomy                     & 0,9924          & 0,9871          & 0,9903          & \textbf{0,9951} & 0,9915          & \textit{0,9966} & 292.0      \\
Volume loss                    & \textbf{0,9171} & 0,9025          & 0,9043          & 0,8961          & 0,9017          & \textit{0,9281} & 294.0      \\
Hiatal hernia                  & 0,9390          & 0,9413          & 0,9469          & \textbf{0,9636} & 0,9467          & \textit{0,9668} & 287.0      \\
Hemidiaphragm elevation        & 0,8928          & 0,8820          & \textbf{0,9149} & 0,8940          & 0,8976          & \textit{0,9338} & 254.0      \\
Pseudonodule                   & 0,6120          & \textbf{0,6696} & 0,5982          & 0,5890          & 0,5446          & \textit{0,6721} & 275.0      \\
Alveolar pattern               & 0,8761          & 0,8771          & 0,8854          & \textbf{0,8949} & 0,8706          & \textit{0,9111} & 248.0      \\
Increased density              & 0,6426          & 0,6411          & 0,6507          & 0,6333          & \textbf{0,6676} & \textit{0,6725} & 239.0      \\
Suture material                & 0,8193          & 0,8203          & 0,8175          & 0,8112          & \textbf{0,8218} & \textit{0,8472} & 210.0      \\
Vertebral anterior compression & \textbf{0,7490} & 0,6958          & 0,7357          & 0,7432          & 0,7340          & \textit{0,7519} & 214.0      \\
Supra aortic elongation        & 0,8646          & 0,8205          & 0,8798          & \textbf{0,8817} & 0,8572          & \textit{0,8939} & 200.0      \\ \midrule 
\textbf{Global}                         & \textbf{0,8184} & 0,8044          & 0,7967          & 0,7804          & 0,7819          & \textit{0,8397} &        \\   \midrule
\end{tabular}}
\end{table}


\begin{tabular}{r|lllll|l|l}  \toprule
                               & DenseNet 201    & EfficientNet    & Inception       & InceptionResnet & Xception        & ensemble        & n\_samples \\ \midrule \midrule
Normal                         & 0,7341          & 0,7066          & \textbf{0,7493} & 0,7230          & 0,7315          & \textit{0,7700} & 34327.0    \\
Copd signs                     & 0,7709          & 0,7609          & 0,7709          & \textbf{0,7928} & 0,7786          & \textit{0,8164} & 13419      \\
Cardiomegaly                   & 0,8990          & \textbf{0,9035} & 0,8896          & 0,8924          & 0,8983          & \textit{0,9227} & 8120       \\
Thoracic cage deformation      & 0,7059          & \textbf{0,7283} & 0,5000          & 0,6754          & 0,7084          & \textit{0,7449} & 7778       \\
Aortic elongation              & 0,8576          & 0,8528          & 0,8419          & 0,8657          & \textbf{0,8661} & \textit{0,8863} & 7436       \\
Infiltrates                    & 0,7943          & \textbf{0,8016} & 0,7912          & 0,7970          & 0,7942          & \textit{0,8265} & 6706       \\
Unchanged                      & 0,6301          & \textbf{0,6364} & 0,6183          & 0,6329          & 0,6311          & \textit{0,6523} & 6487       \\
Chronic changes                & 0,7589          & 0,7539          & 0,7521          & 0,7344          & \textbf{0,7397} & \textit{0,7679} & 4312       \\
Surgery                        & 0,8126          & 0,8147          & 0,7501          & 0,7661          & \textbf{0,8290} & \textit{0,8451} & 3928       \\
atelectasis                    & \textbf{0,7981} & 0,7557          & 0,6982          & 0,7293          & 0,7585          & \textit{0,8039} & 3565       \\
Costophrenic angle blunting    & \textbf{0,8454} & 0,8068          & 0,7583          & 0,7843          & 0,8284          & \textit{0,8636} & 3306       \\
Calcified densities            & 0,7194          & \textbf{0,7510} & 0,5000          & 0,5000          & 0,5000          & \textit{0,7638} & 3253       \\
Vertebral degenerative changes & \textbf{0,7436} & 0,7265          & 0,6764          & 0,7333          & 0,7298          & \textit{0,7507} & 3203       \\
Hilar enlargement              & \textbf{0,7548} & 0,7324          & 0,6991          & 0,7380          & 0,7307          & \textit{0,7653} & 3162       \\
Pleural thickening             & 0,7526          & \textbf{0,7726} & 0,7373          & 0,7435          & 0,7629          & \textit{0,7903} & 3010       \\
Mediastinal enlargement        & 0,7952          & 0,7979          & 0,7742          & 0,7776          & \textbf{0,8219} & \textit{0,8408} & 2813       \\
Air trapping                   & 0,6541          & 0,6686          & 0,5000          & 0,6653          & \textbf{0,6720} & \textit{0,6919} & 2765       \\
Fracture                       & \textbf{0,7490} & 0,7245          & 0,5000          & 0,6399          & 0,7320          & \textit{0,7924} & 2529       \\
Pleural effusion               & \textbf{0,9417} & 0,9269          & 0,9301          & 0,9354          & 0,9367          & \textit{0,9563} & 2436       \\
Granuloma                      & 0,5000          & \textbf{0,7769} & 0,5000          & 0,5000          & 0,5000          & \textit{0,7769} & 2306       \\
Nodule                         & 0,6533          & \textbf{0,6793} & 0,6167          & 0,6430          & 0,6215          & \textit{0,7066} & 1936       \\
Fibrotic band                  & 0,7382          & \textbf{0,7467} & 0,7119          & 0,5000          & 0,7265          & \textit{0,7695} & 1781       \\
Electrical device              & 0,9925          & 0,9918          & 0,9921          & \textbf{0,9938} & 0,9919          & \textit{0,9969} & 1772       \\
Pneumonia                      & 0,8035          & 0,7896          & 0,8039          & \textbf{0,8130} & 0,7990          & \textit{0,8542} & 1652       \\
Aortic atheromatosis           & 0,8340          & 0,8299          & 0,8130          & 0,8400          & \textbf{0,8432} & \textit{0,8662} & 1581       \\
Pseudonodule                   & 0,6930          & \textbf{0,7271} & 0,5000          & 0,5000          & 0,7084          & \textit{0,7587} & 1451       \\
Bronchiectasis                 & 0,7950          & 0,7759          & 0,7891          & \textbf{0,8136} & 0,7786          & \textit{0,8331} & 1430       \\
Hiatal hernia                  & 0,9165          & 0,8915          & 0,9062          & 0,9178          & \textbf{0,9274} & \textit{0,9586} & 1362       \\
Hemidiaphragm elevation        & 0,8145          & 0,8405          & \textbf{0,8415} & 0,8232          & 0,8106          & \textit{0,8901} & 1231       \\
Increased density              & 0,6330          & \textbf{0,6402} & 0,5961          & 0,6092          & 0,6056          & \textit{0,6608} & 1133       \\
Diaphragmatic eventration      & 0,5000          & \textbf{0,7746} & 0,5000          & 0,5000          & 0,5000          & \textit{0,7746} & 757        \\
Volume loss                    & 0,8016          & 0,7762          & \textbf{0,8090} & 0,8142          & 0,7761          & \textit{0,8645} & 684        \\
Adenopathy                     & 0,5000          & \textbf{0,6966} & 0,5000          & 0,5485          & 0,5825          & \textit{0,7152} & 659        \\
Bronchovascular markings       & 0,7124          & 0,7385          & \textbf{0,7769} & 0,7647          & 0,7036          & \textit{0,8016} & 602        \\
Mass                           & 0,7067          & 0,7151          & 0,7438          & 0,7322          & \textbf{0,7456} & \textit{0,8056} & 574        \\
Artificial heart valve         & 0,9688          & 0,9528          & 0,9753          & \textbf{0,9774} & 0,9722          & \textit{0,9805} & 562        \\
Catheter                       & 0,8714          & 0,8740          & 0,8657          & \textbf{0,8775} & 0,8611          & \textit{0,9046} & 545        \\
Suboptimal study               & 0,7432          & 0,6930          & \textbf{0,7537} & 0,6966          & 0,7271          & \textit{0,7840} & 544        \\
Pulmonary fibrosis             & 0,8501          & 0,8340          & 0,8374          & 0,8640          & \textbf{0,8619} & \textit{0,8917} & 523        \\
Heart insufficiency            & 0,8748          & 0,8768          & \textbf{0,8959} & 0,8840          & 0,8703          & \textit{0,9195} & 520        \\
Hypoexpansion                  & 0,8382          & 0,7453          & \textbf{0,8458} & 0,7679          & 0,5000          & \textit{0,9005} & 476        \\
Gynecomastia                   & 0,8517          & 0,8097          & 0,8520          & \textbf{0,8583} & 0,8059          & \textit{0,9165} & 437        \\
Emphysema                      & 0,7798          & 0,7152          & 0,8006          & \textbf{0,8091} & 0,7240          & \textit{0,8618} & 410        \\
Sclerotic bone lesion          & \textbf{0,5057} & 0,5000          & 0,5000          & 0,5000          & 0,5000          & \textit{0,5057} & 352        \\
Fissure thickening             & 0,8163          & 0,8020          & 0,8192          & \textbf{0,8419} & 0,7981          & \textit{0,8913} & 336        \\
Hilar congestion               & 0,7855          & 0,7982          & 0,7905          & 0,8269          & \textbf{0,8076} & \textit{0,8957} & 318        \\
Osteopenia                     & 0,6586          & 0,6881          & 0,6587          & 0,6950          & \textbf{0,7006} & \textit{0,7519} & 318        \\
Tuberculosis                   & 0,8524          & 0,8607          & \textbf{0,8686} & 0,8244          & 0,8053          & \textit{0,9091} & 299        \\
Bullas                         & \textbf{0,7462} & 0,6852          & 0,7387          & 0,7147          & 0,6508          & \textit{0,7773} & 290        \\
Hyperinflated lung             & 0,7155          & 0,6295          & \textbf{0,7192} & 0,6452          & 0,6587          & \textit{0,7283} & 272        \\
Cavitation                     & 0,7803          & 0,8341          & \textbf{0,8555} & 0,7893          & 0,8228          & \textit{0,9341} & 243        \\
Mediastinic lipomatosis        & \textbf{0,6477} & 0,6539          & 0,5000          & 0,5000          & 0,5000          & \textit{0,6813} & 212        \\
Pneumothorax                   & 0,7052          & 0,7170          & \textbf{0,7171} & 0,7206          & 0,6201          & \textit{0,8468} & 210        \\
Vascular redistribution        & \textbf{0,7742} & 0,7522          & 0,7047          & 0,6941          & 0,6670          & \textit{0,8367} & 204        \\ \midrule
\textbf{Global}                         & 0,7559          & \textbf{0,7624} & 0,7279          & 0,7350          & 0,7350          & \textit{0,8128} &     \\     \midrule 
\end{tabular}




\begin{figure}[!h]
\centering
    \begin{subfigure}{0.45\linewidth}
\includegraphics[width=\linewidth]{images/heatmap_v1/normal.pdf} 
    \caption{}
\label{fig:heat1_v1}
    \end{subfigure}\hfill
    \begin{subfigure}{0.45\linewidth}
\includegraphics[width=\linewidth]{images/heatmap_v1/threelabels_cardio.pdf}
    \caption{}
\label{fig:heat2_v1}
    \end{subfigure}

    \begin{subfigure}{0.45\linewidth}
\includegraphics[width=\linewidth]{images/heatmap_v1/cardiome.pdf}
    \caption{}
\label{fig:heat3_v1}
    \end{subfigure}\hfill
    \begin{subfigure}{0.45\linewidth}
\includegraphics[width=\linewidth]{images/heatmap_v1/threelabels_suture.pdf}
    \caption{}
\label{fig:heat4_v1}
    \end{subfigure}
\caption{Heatmaps generated with the ensemble system. a) sample without radiological signs, normal (pink); b) sample with signs of cardiomegaly (purple), pacemaker (dark green) and sternotomy (cyan); c) sample with signs of cardiomegaly; d) sample with signs of pleural effusion (light orange), laminar altelectasis (red), and suture material (green blue).}
    \label{fig:heatmaps_v1}
    \end{figure}
    
    
    
\begin{figure}[h]
  \caption{A picture of a gull.}
  \begin{center}
    \includegraphics[width=\textwidth]{images/30661727075761817007267292459310975718_86nsuj.png}
  \end{center}
\end{figure}

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=\textwidth]{images/3137231742710829928-247610802266403640553_kine6a.png}
  \end{center}
  \caption{A picture of the same gull looking the other way!}
\end{figure}

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.5\textwidth]{images/97965053291113766610970450200683915158_ta7i4n.png}
  \end{center}
  \caption{A picture of the same gull looking the other way!}
\end{figure}

